Optimizing Data Collection in Deep Reinforcement Learning

Reinforcement learning (RL) workloads take a notoriously long time to train due to the large number of samples collected at run-time from simulators. Unfortunately, cluster scale-up approaches remain expensive, and commonly used CPU implementations of simulators induce high overhead when switching back and forth between GPU computations. We explore two optimizations that increase RL data collection efficiency by increasing GPU utilization: (1) GPU vectorization: parallelizing simulation on the GPU for increased hardware parallelism, and (2) simulator kernel fusion: fusing multiple simulation steps to run in a single GPU kernel launch to reduce global memory bandwidth requirements. We find that GPU vectorization can achieve up to $1024\times$ speedup over commonly used CPU simulators. We profile the performance of different implementations and show that for a simple simulator, ML compiler implementations (XLA) of GPU vectorization outperform a DNN framework (PyTorch) by $13.4\times$ by reducing CPU overhead from repeated Python to DL backend API calls. We show that simulator kernel fusion speedups with a simple simulator are $11.3\times$ and increase by up to $1024\times$ as simulator complexity increases in terms of memory bandwidth requirements. We show that the speedups from simulator kernel fusion are orthogonal and combinable with GPU vectorization, leading to a multiplicative speedup.

==> Makefile <==
####################################################################################################
# Latex stuff.
####################################################################################################

DEPENDS :=
STYLE_DIR := 
MAIN_TEX_STEM := rl_optimization_paper
PDF := $(MAIN_TEX_STEM).pdf
MAIN_TEX := $(shell find -name $(MAIN_TEX_STEM).tex)
BIB := $(shell find -name $(MAIN_TEX_STEM).bib)
DEPENDS += $(BIB)
TEX := $(shell find -name '*.tex' | grep -v '/tex_arXiv')
DEPENDS += $(TEX)
FIGS := $(shell find -regextype posix-extended -regex '.*.(pdf|png|svg)' | grep -v $(PDF))
DEPENDS += $(FIGS)
PY := $(shell find -regextype posix-extended -regex '.*.(py)')
STY := $(shell find -regextype posix-extended -regex '.*.(sty)')
DEPENDS += $(STY)
# Make sure we are using virtual environment.
PYTHON := ./venv/bin/python
RUBBER := rubber

.PHONY: clean all arxiv arxiv_clean help

all: $(PDF)

help:
	@echo "$$ make arxiv"
	@echo "  Build uploadable *.tar.gz file for uploading RL-Scope paper to arXiv."
	@echo
	@echo "$$ make"
	@echo "  Build paper PDF."
	@echo
	@echo "$$ make clean"
	@echo "  Delete latex files and paper PDF"

$(PDF): $(MAIN_TEX) $(DEPENDS) Makefile
	$(RUBBER) -f --pdf -s --clean $<
	$(RUBBER) -f --pdf -s $<
	rubber-info --check $<
	@echo "Success!"

arxiv: rl_optimization_paper_arxiv.tar.gz
rl_optimization_paper_arxiv.tar.gz: rl_opt_paper/scripts/package_arxiv.py $(DEPENDS) Makefile
	$(PYTHON) rl_opt_paper/scripts/package_arxiv.py

clean:
	rm -rf *.aux *.bbl *.blg *.log *.pdf *.toc *.snm *.out *.nav tags *.tar.gz *.cut

# Remove same stuff as clean EXCEPT *.bbl to make arxiv happy
# (+ extra *.log.txt files)
arxiv_clean:
	rm -rf *.aux *.blg *.log *.pdf *.toc *.snm *.out *.nav tags *.tar.gz *.cut \
		*.log.txt


==> tex/custom_imports.tex <==


\RequirePackage{caption}
\RequirePackage{subcaption}
\RequirePackage[dvipsnames,prologue]{xcolor}
\RequirePackage{tcolorbox}

\RequirePackage{cleveref}
\crefformat{footnote}{#2\footnotemark[#1]#3}



\RequirePackage{textcomp}

\RequirePackage{centernot}

\RequirePackage{graphbox}

\RequirePackage{listings}
\RequirePackage{tikz}

\usetikzlibrary{arrows}
\usetikzlibrary{shapes}

\RequirePackage[normalem]{ulem}
\RequirePackage{enumitem}
\RequirePackage{siunitx}
\RequirePackage[nomessages]{fp}

\RequirePackage{xspace} 

\RequirePackage{comment} 
